Causal Analysis of the TOPCAT Trial: Spironolactone for Preserved Cardiac Function Heart Failure

We describe the results of applying causal discovery methods on the data from a multi-site clinical trial, on the Treatment of Preserved Cardiac Function Heart Failure with an Aldosterone Antagonist (TOPCAT). The trial was inconclusive, with no clear benefits consistently shown for the whole cohort. However, there were questions regarding the reliability of the diagnosis and treatment protocol for a geographic subgroup of the cohort. With the inclusion of medical context in the form of domain knowledge, causal discovery is used to demonstrate regional discrepancies and to frame the regional transportability of the results. Furthermore, we show that, globally and especially for some subgroups, the treatment has significant causal effects, thus offering a more refined view of the trial results.

==> figures/full_dag.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}[scale=2]

\definecolor{darkgray176}{RGB}{176,176,176}

\begin{axis}[
scaled x ticks=manual:{}{\pgfmathparse{#1}},
scaled y ticks=manual:{}{\pgfmathparse{#1}},
tick align=outside,
x grid style={grid=none},
xmajorticks=false,
xmin=27.26, xmax=1464.74,
xtick style={color=white},
xticklabels={},
y grid style={grid=none},
ymajorticks=false,
ymin=-34.92, ymax=574.92,
ytick style={color=white},
yticklabels={},
extra x tick style={grid=none},
]
\draw[-latex,draw=black!50] (axis cs:780,522) -- (axis cs:677,306);
\draw[-latex,draw=black!50] (axis cs:780,522) -- (axis cs:367,90);
\draw[-latex,draw=black!50] (axis cs:780,522) -- (axis cs:302,18);
\draw[-latex,draw=black!50] (axis cs:780,522) -- (axis cs:465,234);
\draw[-latex,draw=black!50] (axis cs:780,522) -- (axis cs:409,378);
\draw[-latex,draw=black!50] (axis cs:780,522) -- (axis cs:248,450);
\draw[-latex,draw=black!50] (axis cs:780,522) -- (axis cs:1340,450);
\draw[-latex,draw=black!50] (axis cs:780,522) -- (axis cs:619,450);
\draw[-latex,draw=black!50] (axis cs:780,522) -- (axis cs:954,450);
\draw[-latex,draw=black!50] (axis cs:152,522) -- (axis cs:677,306);
\draw[-latex,draw=black!50] (axis cs:152,522) -- (axis cs:264,162);
\draw[-latex,draw=black!50] (axis cs:152,522) -- (axis cs:367,90);
\draw[-latex,draw=black!50] (axis cs:152,522) -- (axis cs:302,18);
\draw[-latex,draw=black!50] (axis cs:152,522) -- (axis cs:465,234);
\draw[-latex,draw=black!50] (axis cs:152,522) -- (axis cs:409,378);
\draw[-latex,draw=black!50] (axis cs:152,522) -- (axis cs:248,450);
\draw[-latex,draw=black!50] (axis cs:677,306) -- (axis cs:264,162);
\draw[-latex,draw=black!50] (axis cs:677,306) -- (axis cs:367,90);
\draw[-latex,draw=black!50] (axis cs:677,306) -- (axis cs:302,18);
\draw[-latex,draw=black!50] (axis cs:677,306) -- (axis cs:465,234);
\draw[-latex,draw=black!50] (axis cs:677,306) -- (axis cs:640,18);
\draw[-latex,draw=black!50] (axis cs:264,162) -- (axis cs:367,90);
\draw[-latex,draw=black!50] (axis cs:264,162) -- (axis cs:302,18);
\draw[-latex,draw=black!50] (axis cs:367,90) -- (axis cs:302,18);
\draw[-latex,draw=black!50] (axis cs:367,90) -- (axis cs:640,18);
\draw[-latex,draw=black!50] (axis cs:465,234) -- (axis cs:264,162);
\draw[-latex,draw=black!50] (axis cs:465,234) -- (axis cs:367,90);
\draw[-latex,draw=black!50] (axis cs:465,234) -- (axis cs:302,18);
\draw[-latex,draw=black!50] (axis cs:465,234) -- (axis cs:640,18);
\draw[-latex,draw=black!50] (axis cs:409,378) -- (axis cs:677,306);
\draw[-latex,draw=black!50] (axis cs:409,378) -- (axis cs:264,162);
\draw[-latex,draw=black!50] (axis cs:409,378) -- (axis cs:367,90);
\draw[-latex,draw=black!50] (axis cs:409,378) -- (axis cs:302,18);
\draw[-latex,draw=black!50] (axis cs:409,378) -- (axis cs:465,234);
\draw[-latex,draw=black!50] (axis cs:409,378) -- (axis cs:640,18);
\draw[-latex,draw=black!50] (axis cs:248,450) -- (axis cs:677,306);
\draw[-latex,draw=black!50] (axis cs:248,450) -- (axis cs:264,162);
\draw[-latex,draw=black!50] (axis cs:248,450) -- (axis cs:367,90);
\draw[-latex,draw=black!50] (axis cs:248,450) -- (axis cs:302,18);
\draw[-latex,draw=black!50] (axis cs:248,450) -- (axis cs:465,234);
\draw[-latex,draw=black!50] (axis cs:248,450) -- (axis cs:409,378);

\draw (axis cs:780,522) node[
  draw=Green, 
  fill=Green!30,
  scale=0.3,
  text=black,
  rotate=0.0,
]{treatment};
\draw (axis cs:152,522) node[
  draw=blue, 
  fill=white,
  scale=0.3,
  text=black,
  rotate=0.0
]{warfarin use};
\draw (axis cs:677,306) node[
  draw=blue, 
  fill=white,
  scale=0.3,
  text=black,
  rotate=0.0
]{Outcome abortedca};
\draw (axis cs:264,162) node[
  draw=blue, 
  fill=white,
  scale=0.3,
  text=black,
  rotate=0.0
]{Outcome anyhosp};
\draw (axis cs:367,90) node[
  draw=blue, 
  fill=white,
  scale=0.3,
  text=black,
  rotate=0.0
]{Outcome cvd death};
\draw (axis cs:302,18) node[
  draw=blue, 
  fill=white,
  scale=0.3,
  text=black,
  rotate=0.0
]{Outcome death};
\draw (axis cs:465,234) node[
  draw=blue, 
  fill=white,
  scale=0.3,
  text=black,
  rotate=0.0
]{Outcome hfhosp};
\draw (axis cs:409,378) node[
  draw=blue, 
  fill=white,
  scale=0.3,
  text=black,
  rotate=0.0
]{Outcome mi};
\draw (axis cs:640,18) node[
  draw=blue, 
  fill=white,
  scale=0.3,
  text=black,
  rotate=0.0
]{Outcome primary ep};
\draw (axis cs:248,450) node[
  draw=blue, 
  fill=white,
  scale=0.3,
  text=black,
  rotate=0.0
]{Outcome stroke};
\draw (axis cs:1340,450) node[
  draw=blue, 
  fill=white,
  scale=0.3,
  text=black,
  rotate=0.0
]{hyperkalemia side effect discontinued};
\draw (axis cs:619,450) node[
  draw=blue, 
  fill=white,
  scale=0.3,
  text=black,
  rotate=0.0
]{potassium side effect discontinued};
\draw (axis cs:954,450) node[
  draw=blue, 
  fill=white,
  scale=0.3,
  text=black,
  rotate=0.0
]{renal function side effect discontinued};
\end{axis}
\end{tikzpicture}

